A Frustratingly Easy Approach for Entity and Relation Extraction

End-to-end relation extraction aims to identify named entities and extract relations between them. Most recent work models these two subtasks jointly, either by casting them in one structured prediction framework, or performing multi-task learning through shared representations. In this work, we present a simple pipelined approach for entity and relation extraction, and establish the new state-of-the-art on standard benchmarks (ACE04, ACE05 and SciERC), obtaining a 1.7%-2.8% absolute improvement in relation F1 over previous joint models with the same pre-trained encoders. Our approach essentially builds on two independent encoders and merely uses the entity model to construct the input for the relation model. Through a series of careful examinations, we validate the importance of learning distinct contextual representations for entities and relations, fusing entity information early in the relation model, and incorporating global context. Finally, we also present an efficient approximation to our approach which requires only one pass of both entity and relation encoders at inference time, achieving an 8-16$\times$ speedup with a slight reduction in accuracy.

==> 7_ethical.tex <==
\section*{Ethical Considerations}
The datasets (ACE04, ACE05, and SciERC) applied in our research are collected from newswire, broadcast news, or published scientific papers.
They are all publicly available and do not contain privacy-sensitive data.
We think there are no privacy or safety concerns about our research.
On the other hand, our model may produce biased predictions, if it is trained on a biased training set.
For example, our entity model may be more likely to classify the mention ``Boeing'' to be a company instead of a person, if the model is trained on a corpus mainly containing aircraft news.
We could also imagine that some gender or race biases can also be introduced by training the model on a biased dataset.
We believe this biased-prediction problem is not specific to our research and already existed before our research, and it should be broadly addressed by the community in the future.

